Disparate Effect Of Missing Mediators On Transportability of Causal Effects

Transported mediation effects provide an avenue to understand how upstream interventions (such as improved neighborhood conditions like green spaces) would work differently when applied to different populations as a result of factors that mediate the effects. However, when mediators are missing in the population where the effect is to be transported, these estimates could be biased. We study this issue of missing mediators, motivated by challenges in public health, wherein mediators can be missing, not at random. We propose a sensitivity analysis framework that quantifies the impact of missing mediator data on transported mediation effects. This framework enables us to identify the settings under which the conditional transported mediation effect is rendered insignificant for the subgroup with missing mediator data. Specifically, we provide the bounds on the transported mediation effect as a function of missingness. We then apply the framework to longitudinal data from the Moving to Opportunity Study, a large-scale housing voucher experiment, to quantify the effect of missing mediators on transport effect estimates of voucher receipt, an upstream intervention on living location, in childhood on subsequent risk of mental health or substance use disorder mediated through parental health across sites. Our findings provide a tangible understanding of how much missing data can be withstood for unbiased effect estimates.

==> notes.tex <==

% Code: https://code.nimahejazi.org/ser2022_mediation_workshop/additional-topics-of-interest.html#mediation-with-time-varying-treatments-mediators-and-covariates


We first present the results of the effect of ‘taking two or more anti-hypertensives on average diastolic blood pressure. 
% Then, we present the results of the effect of ‘taking beta blockers and diuretics’ on average systolic blood pressure.
The treatment is defined from reported prescription drug use, and those drugs primary use classes. We include the following pre-treatment variables as covariates: An indicator variable for whether the respondent is female, an indicator for whether the respondent is non-Hispanic white, an indicator for whether she or he is black, an indicator for whether she or he is Hispanic, age (in months), household size, number of years of education completed, indicators for whether she or he is married, whether s\/he is widowed
% d, whether s\/he is separated (using never married as a baseline category), logged annual household income, pack years (number of packs smoked everyday multiplied by number of years smoked), body mass index((mass (lb) \/height (in)2)× 703), radial pulse rate (beats \/min), sodium intake (mg), potassium intake (mg), sodium–potassium ratio, an indicator for whether she or he has health insurance, and finally the frequency of meeting with friends or relatives per year. We consider "alcohol intake (g)" as the mediator which is perturbed to include missingness for generating a semi-synthetic setup. 

% \section{Introduction skeleton}
% \begin{itemize}
%     \item Background on transporting causal effects across populations.
%     \item Describe how missing mediators can pose a challenge to estimating valid significant estimates of causal effects.
%     \item Motivate the problem of missing mediators from public health, specifically, the missingness mechanism introduced by not reporting behaviors like alcohol consumption and missing data about opioid consumption leading to opioid-related deaths. 
%     \item Introduce the sensitivity framework for missing mediators and highlight how this sensitivity framework is different than previous sensitivity frameworks proposed for unobserved confounders.
%     \item Brief description of theoretical and empirical results on simulated data and NHANES.
% \end{itemize}




\cut{\section{Real-world datasets and Journals}
Datasets
\begin{enumerate}
    \item NHANES III (Kaggle code: https://www.kaggle.com/datasets/cdc/national-health-and-nutrition-examination-survey?select=examination.csv)
\end{enumerate}
Journals
\begin{enumerate}
    \item Statistics in Medicine {\citep{dorie2016flexible}}
    \item Plos One (https://journals.plos.org/plosone/)
    \item Epidemiologic Methods (https://www.degruyter.com/journal/key/em/html?lang=en\#overview)
\end{enumerate}
}
